Optimization with Non-Differentiable Constraints with Applications to Fairness, Recall, Churn, and Other Goals

We show that many machine learning goals, such as improved fairness metrics, can be expressed as constraints on the model's predictions, which we call rate constraints. We study the problem of training non-convex models subject to these rate constraints (or any non-convex and non-differentiable constraints). In the non-convex setting, the standard approach of Lagrange multipliers may fail. Furthermore, if the constraints are non-differentiable, then one cannot optimize the Lagrangian with gradient-based methods. To solve these issues, we introduce the proxy-Lagrangian formulation. This new formulation leads to an algorithm that produces a stochastic classifier by playing a two-player non-zero-sum game solving for what we call a semi-coarse correlated equilibrium, which in turn corresponds to an approximately optimal and feasible solution to the constrained optimization problem. We then give a procedure which shrinks the randomized solution down to one that is a mixture of at most $m+1$ deterministic solutions, given $m$ constraints. This culminates in algorithms that can solve non-convex constrained optimization problems with possibly non-differentiable and non-convex constraints with theoretical guarantees. We provide extensive experimental results enforcing a wide range of policy goals including different fairness metrics, and other goals on accuracy, coverage, recall, and churn.

==> figures/fig-counterexample.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
  %
  \vspace{-3em}
  %
  \centering
  %
  \includegraphics[width=0.45\textwidth]{images/counterexample}
  %
  \caption{
    %
    %\begin{titled-paragraph}{Nonexistence of a pure Nash equilibrium of the
    %Lagrangian game}
    %
    The plotted rectangular region is the domain \Parameters, the contours are
    those of the \emph{strictly concave} minimization objective function
    \objective, and the shaded triangle is the feasible region determined by
    the three linear inequality constraints $\constraint{1}, \dots,
    \constraint{3}$. The red dot is the optimal feasible point.
    %
    The Lagrangian $\lagrangian\left(\parameters, \multipliers\right)$ is
    strictly concave in \parameters for any choice of \multipliers, so the
    optimal choice(s) for the \parameters-player will always lie on the four
    corners of the plotted rectangle. However, these points are infeasible, and
    therefore suboptimal for the \multipliers-player
    %
    (assuming that $\multipliers \in \Multipliers = \R_+^3$).
    %
    %\end{titled-paragraph}
    %
  }
  %
  \label{fig:counterexample}
  \vspace{-1.5em}
  %
\end{wrapfigure}


==> images/alg-oracle-lagrangian.tex <==
\begin{algorithm*}[t]

\begin{pseudocode}
\codename $\mbox{OracleLagrangian}\left( \Radius \in \R_+, \lagrangian : \Parameters \times \Multipliers \rightarrow \R, \oracle : \left(\Parameters \rightarrow \R\right) \rightarrow \Parameters, T \in \N, \eta_{\multipliers} \in \R_+ \right)$: \\
%
\codeline Initialize $\multipliers^{(1)} = 0$ \\
\codeline For $t \in \indices{T}$: \\
\codeline \> Let $\parameters^{(t)} = \oracle\left( \lagrangian\left(\cdot,\multipliers^{(t)}\right) \right)$ \codecomment{Oracle optimization} \\
\codeline \> Let $\stochasticgrad^{(t)}_{\multipliers}$ be a gradient of $\lagrangian\left(\parameters^{(t)},\multipliers^{(t)}\right)$ \wrt $\multipliers$ \\
\codeline \> Update $\multipliers^{(t+1)} = \Pi_{\Multipliers}\left( \multipliers^{(t)} + \eta_{\multipliers} \stochasticgrad^{(t)}_{\multipliers} \right)$ \codecomment{Projected gradient update} \\
\codeline Return $\parameters^{(1)},\dots,\parameters^{(T)}$ and $\multipliers^{(1)},\dots,\multipliers^{(T)}$
%
\end{pseudocode}

\caption{
  %
  Optimizes the Lagrangian formulation (\defref{lagrangian}) in the non-convex
  setting via the use of an approximate Bayesian optimization oracle $\oracle$
  (\defref{oracle}) for the $\parameters$-player.
  %
  The parameter $\Radius$ is the radius of the Lagrange multiplier space
  $\Multipliers \defeq \left\{ \multipliers \in \R_+^{\numconstraints} :
  \norm{\multipliers}_1 \le \Radius \right\}$, and the function
  $\Pi_{\Multipliers}$ projects its argument onto $\Multipliers$ \wrt the
  Euclidean norm.
  %
}

\label{alg:oracle-lagrangian}

\end{algorithm*}


==> images/alg-oracle-proxy-lagrangian.tex <==
\begin{algorithm*}[t]

\begin{pseudocode}
\codename $\mbox{OracleProxyLagrangian}\left( \lagrangian_{\parameters}, \lagrangian_{\multipliers} : \Parameters \times \Delta^{\numconstraints+1} \rightarrow \R, \oracle : \left(\Parameters \rightarrow \R\right) \rightarrow \Parameters, T \in \N, \eta_{\multipliers} \in \R_+ \right)$: \\
%
\codeline Initialize $\matrixmultipliers^{(1)} \in \R^{\left(\numconstraints + 1\right) \times \left(\numconstraints + 1\right)}$ with $\matrixmultipliers_{i,j} = 1 / \left(\numconstraints+1\right)$ \\
\codeline For $t \in \indices{T}$: \\
\codeline \> Let $\multipliers^{(t)} = \fix \matrixmultipliers^{(t)}$ \codecomment{Stationary distribution of $\matrixmultipliers^{(t)}$} \\
\codeline \> Let $\parameters^{(t)} = \oracle\left( \lagrangian_{\parameters}\left(\cdot,\multipliers^{(t)}\right) \right)$ \codecomment{Oracle optimization} \\
\codeline \> Let $\stochasticgrad^{(t)}_{\multipliers}$ be a gradient of $\lagrangian_{\multipliers}\left(\parameters^{(t)},\multipliers^{(t)}\right)$ \wrt $\multipliers$ \\
\codeline \> Update $\tilde{\matrixmultipliers}^{(t+1)} = \matrixmultipliers^{(t)} \elementwiseproduct \elementwiseexp\left( \eta_{\multipliers} \stochasticgrad^{(t)}_{\multipliers} \left( \multipliers^{(t)} \right)^T \right)$ \codecomment{$\elementwiseproduct$ and $\elementwiseexp$ are element-wise} \\
\codeline \> Project $\matrixmultipliers^{(t+1)}_{:,i} = \tilde{\matrixmultipliers}^{(t+1)}_{:,i} / \norm{\tilde{\matrixmultipliers}^{(t+1)}_{:,i}}_1$ for $i\in\indices{\numconstraints+1}$ \codecomment{Column-wise projection}  \\
\codeline Return $\parameters^{(1)},\dots,\parameters^{(T)}$ and $\multipliers^{(1)},\dots,\multipliers^{(T)}$
%
\end{pseudocode}

\caption{
  %
  Optimizes the proxy-Lagrangian formulation (\defref{proxy-lagrangians}) in
  the non-convex setting via the use of an approximate Bayesian optimization
  oracle $\oracle$ (\defref{oracle}, but with $\proxyconstraint{i}$s instead of
  $\constraint{i}$s in the linear combination defining $f$) for the
  $\parameters$-player, with the $\multipliers$-player minimizing swap regret.
  %
  The $\fix \matrixmultipliers$ operation on line $3$ results in a stationary
  distribution of $\matrixmultipliers$ (\ie a $\multipliers \in \Multipliers$
  such that $\matrixmultipliers \multipliers = \multipliers$, which can be
  derived from the top eigenvector).
  %
}

\label{alg:oracle-proxy-lagrangian}

\end{algorithm*}


==> images/alg-stochastic-lagrangian.tex <==
\begin{algorithm*}[t]

\begin{pseudocode}
\codename $\mbox{StochasticLagrangian}\left( \Radius \in \R_+, \lagrangian : \Parameters \times \Multipliers \rightarrow \R, T \in \N, \eta_{\parameters}, \eta_{\multipliers} \in \R_+ \right)$: \\
%
\codeline Initialize $\parameters^{(1)} = 0$, $\multipliers^{(1)} = 0$ \codecomment{Assumes $0 \in \Parameters$} \\
\codeline For $t \in \indices{T}$: \\
\codeline \> Let $\stochasticsubgrad^{(t)}_{\parameters}$ be a stochastic subgradient of $\lagrangian\left(\parameters^{(t)},\multipliers^{(t)}\right)$ \wrt $\parameters$ \\
\codeline \> Let $\stochasticgrad^{(t)}_{\multipliers}$ be a stochastic gradient of $\lagrangian\left(\parameters^{(t)},\multipliers^{(t)}\right)$ \wrt $\multipliers$ \\
\codeline \> Update $\parameters^{(t+1)} = \Pi_{\Parameters}\left( \parameters^{(t)} - \eta_{\parameters} \stochasticsubgrad^{(t)}_{\parameters} \right)$ \codecomment{Projected SGD updates \dots} \\
\codeline \> Update $\multipliers^{(t+1)} = \Pi_{\Multipliers}\left( \multipliers^{(t)} + \eta_{\multipliers} \stochasticgrad^{(t)}_{\multipliers} \right)$ \codecomment{\;\;\;\;\dots} \\
\codeline Return $\parameters^{(1)},\dots,\parameters^{(T)}$ and $\multipliers^{(1)},\dots,\multipliers^{(T)}$
%
\end{pseudocode}

\caption{
  %
  Optimizes the Lagrangian formulation (\defref{lagrangian}) in the convex
  setting.
  %
  The parameter $\Radius$ is the radius of the Lagrange multiplier space
  $\Multipliers \defeq \left\{ \multipliers \in \R_+^{\numconstraints} :
  \norm{\multipliers}_1 \le \Radius \right\}$, and the functions
  $\Pi_{\Parameters}$ and $\Pi_{\Multipliers}$ project their arguments onto
  $\Parameters$ and $\Multipliers$ (respectively) \wrt the Euclidean norm.
  %
}

\label{alg:stochastic-lagrangian}

\end{algorithm*}


==> images/alg-stochastic-proxy-lagrangian.tex <==
\begin{algorithm*}[t]

\begin{pseudocode}
%
\codename $\mbox{StochasticProxyLagrangian}\left(\lagrangian_{\parameters}, \lagrangian_{\multipliers} : \Parameters \times \Delta^{\numconstraints+1} \rightarrow \R, T \in \N, \eta_{\parameters}, \eta_{\multipliers} \in \R_+ \right)$: \\
%
\codeline Initialize $\parameters^{(1)} = 0$ \codecomment{Assumes $0 \in \Parameters$} \\
\codeline Initialize $\matrixmultipliers^{(1)} \in \R^{\left(\numconstraints + 1\right) \times \left(\numconstraints + 1\right)}$ with $\matrixmultipliers_{i,j} = 1 / \left(\numconstraints+1\right)$ \\
\codeline For $t \in \indices{T}$: \\
\codeline \> Let $\multipliers^{(t)} = \fix \matrixmultipliers^{(t)}$ \codecomment{Stationary distribution of $\matrixmultipliers^{(t)}$} \\
\codeline \> Let $\stochasticsubgrad^{(t)}_{\parameters}$ be a stochastic subgradient of $\lagrangian_{\parameters}\left(\parameters^{(t)},\multipliers^{(t)}\right)$ \wrt $\parameters$ \\
\codeline \> Let $\stochasticgrad^{(t)}_{\multipliers}$ be a stochastic gradient of $\lagrangian_{\multipliers}\left(\parameters^{(t)},\multipliers^{(t)}\right)$ \wrt $\multipliers$ \\
\codeline \> Update $\parameters^{(t+1)} = \Pi_{\Parameters}\left( \parameters^{(t)} - \eta_{\parameters} \stochasticsubgrad^{(t)}_{\parameters} \right)$ \codecomment{Projected SGD update} \\
\codeline \> Update $\tilde{\matrixmultipliers}^{(t+1)} = \matrixmultipliers^{(t)} \elementwiseproduct \elementwiseexp\left( \eta_{\multipliers} \stochasticgrad^{(t)}_{\multipliers} \left( \multipliers^{(t)} \right)^T \right)$ \codecomment{$\elementwiseproduct$ and $\elementwiseexp$ are element-wise} \\
\codeline \> Project $\matrixmultipliers^{(t+1)}_{:,i} = \tilde{\matrixmultipliers}^{(t+1)}_{:,i} / \norm{\tilde{\matrixmultipliers}^{(t+1)}_{:,i}}_1$ for $i\in\indices{\numconstraints+1}$ \codecomment{Column-wise projection} \\
\codeline Return $\parameters^{(1)},\dots,\parameters^{(T)}$ and $\multipliers^{(1)},\dots,\multipliers^{(T)}$
%
\end{pseudocode}

\caption{
  %
  Optimizes the proxy-Lagrangian formulation (\defref{proxy-lagrangians}) in
  the convex setting, with the $\parameters$-player minimizing external regret,
  and the $\multipliers$-player minimizing swap regret.
  %
  The $\fix \matrixmultipliers$ operation on line $3$ results in a stationary
  distribution of $\matrixmultipliers$ (\ie a $\multipliers \in \Multipliers$
  such that $\matrixmultipliers \multipliers = \multipliers$, which can be
  derived from the top eigenvector).
  %
  The function $\Pi_{\Parameters}$ projects its argument onto $\Parameters$
  \wrt the Euclidean norm.
  %
}

\label{alg:stochastic-proxy-lagrangian}

\end{algorithm*}


==> images/fig-counterexample.tex <==
\begin{wrapfigure}{R}{0.5\textwidth}
  %
  \vspace{-3em}
  %
  \centering
  %
  \includegraphics[width=0.45\textwidth]{images/counterexample}
  %
  \caption{
    %
    %\begin{titled-paragraph}{Nonexistence of a pure Nash equilibrium of the
    %Lagrangian game}
    %
    The plotted rectangular region is the domain \Parameters, the contours are
    those of the \emph{strictly concave} minimization objective function
    \objective, and the shaded triangle is the feasible region determined by
    the three linear inequality constraints $\constraint{1}, \dots,
    \constraint{3}$. The red dot is the optimal feasible point.
    %
    The Lagrangian $\lagrangian\left(\parameters, \multipliers\right)$ is
    strictly concave in \parameters for any choice of \multipliers, so the
    optimal choice(s) for the \parameters-player will always lie on the four
    corners of the plotted rectangle. However, these points are infeasible, and
    therefore suboptimal for the \multipliers-player
    %
    (assuming that $\multipliers \in \Multipliers = \R_+^3$).
    %
    %\end{titled-paragraph}
    %
  }
  %
  \label{fig:counterexample}
  \vspace{-1.5em}
  %
\end{wrapfigure}


==> images/tab-experiments-adult.tex <==
\begin{table*}[t]

\caption{
  %
  Support sizes, test error rates, and ``equal opportunity'' values for the
  experiments of \appref{experiments:adult}. For the constraints, each reported
  number is the ratio of the positive prediction rate on positively-labeled
  members of the protected class, to the positive prediction rate on the set of
  all positively-labeled data. The constraints attempt to force this ratio to
  be at least $95\%$---quantities lower than this threshold violate the
  constraint, and are marked in \textbf{bold}.
  %
  Each row of the ``Testing'' table has a matching row in the ``Training''
  table, which contains the training set results for the \emph{same
  experiment}---the table was only split to fit on the page.
  %
}

\begin{center}
%
\begin{tabular}{r|c|cccc}
  %
  \hline
  %
  & \multicolumn{5}{c}{Testing} \\
  %
  & Error & Female & Male & Black & White \\
  %
  \hline
  %
  Baseline ($\parameters^{(T)}$) &
  14.2\% & \textbf{89.5\%} & 102\% & \textbf{81.6\%} & 101\% \\
  %
  Lagrangian ($\bar{\parameters}$) &
  16.3\% & 114\% & 97.5\% & 126\% & 99.8\% \\
  %
  Lagrangian (LP) &
  15.5\% & 106\% & 99.0\% & 111\% & 101\% \\
  %
  Proxy ($\bar{\parameters}$) &
  14.4\% & \textbf{94.1\%} & 101\% & \textbf{94.9\%} & 100\% \\
  %
  Proxy (LP) &
  14.2\% & \textbf{94.4\%} & 101\% & \textbf{94.9\%} & 100\% \\
  %
  \hline
  %
\end{tabular}
%
\end{center}

\begin{center}
%
\begin{tabular}{r|cccc|c}
  %
  \hline
  %
  & \multicolumn{4}{c|}{Training} & \\
  %
  & Female & Male & Black & White & Support \\
  %
  \hline
  %
  Baseline ($\parameters^{(T)}$) &
  \textbf{88.9\%} & 102\% & \textbf{82.8\%} & 101\% &
  1 \\
  %
  Lagrangian ($\bar{\parameters}$) &
  113\% & 97.8\% & 121\% & 99.7\% &
  100 \\
  %
  Lagrangian (LP) &
  104\% & 99.4\% & 105\% & 101\% &
  3 \\
  %
  Proxy ($\bar{\parameters}$) &
  \textbf{94.7\%} & 101\% & \textbf{94.5\%} & 100\% &
  100 \\
  %
  Proxy (LP) &
  95.0\% & 101\% & 95.0\% & 100\% &
  3 \\
  %
  \hline
  %
\end{tabular}
%
\end{center}

\label{tab:experiments-adult}

\end{table*}


==> images/tab-experiments-mnist.tex <==
\begin{table*}[t]

\caption{
  %
  Error rates on the experiments of \appref{experiments:mnist}. The the columns
  correspond to the four corrupted datasets of \citet{Chen:2017}.
  %
}

\begin{center}
%
\begin{tabular}{r|cccc|cccc}
  %
  \hline
  %
  & \multicolumn{4}{c|}{Testing} & \multicolumn{4}{c}{Training} \\
  %
  & Set 1 & Set 2 & Set 3 & Set 4 &
  Set 1 & Set 2 & Set 3 & Set 4\\
  %
  \hline
  %
  Baseline ($\bar{\parameters}$) &
  2.58 & 2.66 & 2.01 & 2.52 &
  1.06 & 1.45 & 0.43 & 1.10 \\
  %
  Baseline ($\parameters^{(T)}$) &
  1.77 & 1.92 & 1.77 & 1.75 &
  0.04 & 0.40 & 0.01 & 0.08 \\
  %
  Lagrangian ($\bar{\parameters}$) &
  2.04 & 2.15 & 1.96 & 2.04 &
  0.42 & 0.70 & 0.30 & 0.49 \\
  %
  Lagrangian (LP) &
  1.66 & 1.67 & 1.63 & 1.62 &
  0.00 & 0.01 & 0.00 & 0.00 \\
  %
  \hline
  %
\end{tabular}
%
\end{center}

\label{tab:experiments-mnist}

\end{table*}

